SEAM: Shortcut-Aware Real-Time Detection of Scripted vs. Spontaneous Speech for Interview Guardrails

Scripted vs spontaneous speech detection is appealing for interview guardrails, but benchmark performance can be inflated by shortcuts tied to corpus identity, channel conditions, and recording artifacts rather than speaking style itself. We present SEAM, a shortcut-aware framework for real-time scriptedness detection that combines uniform preprocessing, seam-aware sampling, non-speech augmentation, and a compact DistilHuBERT backbone. With 8s windows, the model achieves 0.971 +- 0.004 ROC-AUC on an external interview-domain evaluation set. Removing the shortcut-prevention components improves internal held-out metrics but sharply reduces external performance, indicating shortcut learning. Post-training quantization reduces the model footprint to 41.8MB with little loss in external performance. The results demonstrate that robust real-time scriptedness detection depends not only on the backbone, but on shortcut-aware data design and evaluation. We release code and model checkpoints.

==> old_results.tex <==
\section{Results}
% VSEVOLOD 03/01/26 UPDATED
\subsection{Reported results}
Using the selected configuration (DistilHuBERT, 8\,s windows, top-1 transformer layer unfrozen, noise bank enabled), we train for three epochs and report mean and standard deviation across three seeds on both the LOCO-lite splits and the proprietary interview-domain evaluation set in Table~\ref{tab:final}. 

\begin{table}[H]
\centering
\caption{Final model (DistilHuBERT tr1, 8\,s, 3 epochs). Primary reported results.}
\label{tab:final}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
Seed & Eval Acc & Eval AUC & Test Acc & Test AUC & Ext Acc & Ext AUC \\
\midrule
1337 & 0.9690 & 0.9820 & 0.9639 & 0.9781 & 0.9540 & 0.9725 \\
1338 & 0.9602 & 0.9762 & 0.9548 & 0.9715 & 0.9431 & 0.9669 \\
1339 & 0.9728 & 0.9835 & 0.9681 & 0.9802 & 0.9580 & 0.9745 \\
\midrule
\tikzmarknode{meanL}{mean} & 0.9673 & 0.9806 & 0.9623 & 0.9766 & 0.9517 & \tikzmarknode{meanR}{0.9713} \\
\noalign{%
\begin{tikzpicture}[overlay,remember picture]
\draw[densely dotted, rounded corners, line width=1.0pt]
  ([xshift=-2pt,yshift=3pt]meanL.north west) rectangle
  ([xshift= 2pt,yshift=-2pt]meanR.south east);
\end{tikzpicture}%
}
std  & 0.0065 & 0.0039 & 0.0068 & 0.0045 & 0.0077 & 0.0039 \\
\bottomrule
\end{tabular*}
\end{table}

% VSEVOLOD 03/01/26 UPDATED
\subsection{Window-length selection}
Two-second windows miss phrase-level cues such as intonation arcs, hesitation patterns, and local timing structure, and performance drops accordingly. Performance improves substantially from 2\,s to 8\,s, with 8\,s giving the strongest held-out and interview-domain results. Moving to 12\,s remains competitive but adds latency and yields a small decline in AUC, likely because longer windows contain more silence and are more sensitive to window-to-utterance alignment.

Figure~\ref{fig:window_test} shows the test curves, and Table~\ref{tab:win_ablation} summarizes the best checkpoint per window length.

\begin{figure*}[t]
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_window_test_acc.png}
  \end{minipage}\hfill
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_window_test_auc.png}
  \end{minipage}
  \caption{Window-length sweep: test Accuracy (left) and test ROC-AUC (right) versus training step.}
  \label{fig:window_test}
\end{figure*}

\begin{table}[t]
\centering
\caption{Window-length ablation (DistilHuBERT, unfreeze top-1 transformer, noise bank enabled). ``Ext'' is proprietary interview audio.}
\label{tab:win_ablation}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}crcccc}
\toprule
Win(s) & Step & Test Acc & Test AUC & Ext Acc & Ext AUC \\
\midrule
2  & 120 & 0.7229 & 0.7739 & 0.6572 & 0.7485 \\
4  & 120 & 0.8629 & 0.8889 & 0.8067 & 0.8646 \\
8  & 120 & \textbf{0.8949} & \textbf{0.9287} & \textbf{0.8527} & \textbf{0.8991} \\
12 & 120 & 0.8786 & 0.9067 & 0.8349 & 0.8813 \\
\bottomrule
\end{tabular*}
\end{table}

% VSEVOLOD 03/01/26 UPDATED
\subsection{How much to unfreeze?}
Table~\ref{tab:unfreeze_ablation} shows that unfreezing only the top transformer layer gives the best out-of-domain results. Unfreezing more layers improves adaptation capacity, but that extra flexibility does not translate into better cross-corpus generalization here. Best checkpoints are selected by eval AUC within each setting.

\begin{table}[t]
\centering
\caption{Unfreezing ablation (8\,s windows). Best checkpoint per setting, selected by eval AUC.}
\label{tab:unfreeze_ablation}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc}
\toprule
Setting & Step & Eval AUC & Test Acc & Test AUC \\
\midrule
head & 72  & 0.7799 & 0.7078 & 0.7625 \\
tr1  & 120 & \textbf{0.9550} & \textbf{0.8949} & \textbf{0.9287} \\
tr2  & 120 & 0.9296 & 0.8502 & 0.9031 \\
cnn2 & 72  & 0.7631 & 0.6887 & 0.7354 \\
\bottomrule
\end{tabular*}
\end{table}

\begin{figure*}[t]
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_unfreeze_test_acc.png}
  \end{minipage}\hfill
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_unfreeze_test_auc.png}
  \end{minipage}
  \caption{Unfreezing sweep (8\,s): test Accuracy (left) and test ROC-AUC (right) versus training step.}
  \label{fig:unfreeze}
\end{figure*}

% VSEVOLOD 03/01/26 NEW SECTION
\subsection{Shortcut-prevention ablation}
To isolate the effect of our shortcut-prevention methods, we run a one-epoch ablation at 8\,s windows with DistilHuBERT tr1 while keeping uniform preprocessing enabled and toggling only the noise bank and seam-aware sampling flags. Table~\ref{tab:shortcut_ablation} reports the final checkpoint at 120 steps, and Figure~\ref{fig:shortcut_ablation} shows eval-domain and external-domain AUC over training.

Disabling the noise bank, and especially disabling both safeguards together, improves eval and test AUC inside the LOCO-lite protocol, but sharply degrades interview-domain transfer. This suggests that the apparent in-protocol gains come from reintroducing corpus- or channel-dependent shortcuts rather than learning more stable cues. Seam-aware sampling has a smaller effect than the noise bank on held-out-corpus metrics, but it does improve robustness on the external interview set.

\begin{table}[t]
\centering
\caption{Shortcut-prevention ablation at 8\,s (DistilHuBERT tr1, 1 epoch, 120 steps). Uniform preprocessing remains enabled; only the noise bank and seam-aware sampling flags are changed.}
\label{tab:shortcut_ablation}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc}
\toprule
Setting & Eval AUC & Test AUC & Ext Acc & Ext AUC \\
\midrule
baseline on            & 0.9550 & 0.9287 & \textbf{0.8527} & \textbf{0.8991} \\
seam off               & 0.9638 & 0.9328 & 0.8179 & 0.8674 \\
noise off              & 0.9792 & 0.9491 & 0.7089 & 0.7518 \\
noise off + seam off   & \textbf{0.9848} & \textbf{0.9557} & 0.6882 & 0.7324 \\
\bottomrule
\end{tabular*}
\end{table}

\begin{figure*}[t]
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_shortcut_eval_auc.png}
  \end{minipage}\hfill
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_shortcut_ext_auc.png}
  \end{minipage}
  \caption{Shortcut-prevention ablation: eval AUC (left) and external interview AUC (right) versus training step. Higher in-protocol AUC without shortcut defenses does not translate to better external transfer.}
  \label{fig:shortcut_ablation}
\end{figure*}


\subsection{Backbone screening (frozen encoders)}
We first run a fixed-budget backbone screening to choose an encoder; these numbers are not the primary results. Table~\ref{tab:auc} summarizes LOCO-lite ROC-AUC for frozen encoders trained only with an MLP head.

We compare:
\texttt{ntu-spml/distilhubert},
\texttt{OthmaneJ/distil-wav2vec2},
\texttt{facebook/hubert-base-ls960},
\texttt{facebook/wav2vec2-base-960h},
\texttt{microsoft/wavlm-base-plus}.

\begin{table}[t]
\centering
\caption{Backbone screening: LOCO-lite ROC-AUC with frozen encoder + MLP head (batch size 256, 4 shards per class, 120 steps, 12\,s windows). Used for model selection.}
\label{tab:auc}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccc}
\toprule
Backbone & Fold 1 & Fold 2 & Avg. \\
\midrule
DistilHuBERT (ntu-spml) & 0.839 & 0.859 & 0.849 \\
Distil-wav2vec2 (OthmaneJ) & 0.817 & 0.827 & 0.822 \\
HuBERT Base (facebook) & 0.862 & 0.873 & 0.868 \\
wav2vec2 Base (facebook) & 0.863 & 0.873 & 0.868 \\
WavLM Base+ (microsoft) & \textbf{0.889} & \textbf{0.900} & \textbf{0.895} \\
\bottomrule
\end{tabular*}
\end{table}

We use WavLM Base+ as a reference upper bound, but move forward with DistilHuBERT because the gap in AUC is modest while the footprint and latency are far lower (Section~\ref{sec:eff}).

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{fig_backbone_tradeoff.png}
  \caption{Backbone selection tradeoff between out-of-domain quality and deployment cost. DistilHuBERT is not the absolute AUC leader, but it lies on a favorable quality-efficiency frontier for real-time use.}
  \label{fig:backbone_tradeoff}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{fig_backbone_auc_vs_step.png}
  \caption{Backbone screening: out-of-domain ROC-AUC versus training step.}
  \label{fig:backbone}
\end{figure}

% VSEVOLOD 03/01/26 NEW SECTION
\subsection{Quantized deployment variants}
To assess deployment under real memory budgets, we benchmark post-training quantized variants of the final model on an NVIDIA L4 GPU using the external interview evaluation setting (8\,s windows, batch size 64). We compare a baseline CUDA automatic mixed precision (AMP) run against 8-bit and 4-bit quantized variants. Latencies are averaged across three runs and reported separately for GPU forward-pass compute, inference end-to-end latency including host/device transfers, and full pipeline latency.

Quantization substantially reduces the memory footprint from 90.37\,MB under AMP to 48.74\,MB with INT8 and 41.80\,MB with INT4. This compression does not materially degrade external performance: all three variants achieve nearly identical external accuracy and ROC-AUC, with the INT4 model showing the highest observed AUC.

\begin{table}[t]
\centering
\caption{Quantized deployment benchmark on NVIDIA L4 (external evaluation, 8\,s windows, batch size 64, 3 runs).}
\label{tab:quant}
\scriptsize
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
Precision & VRAM (MB) & Ext Acc (\%) & Ext AUC & GPU Fwd (ms/win) & Infer E2E (ms/win) & Full Pipe (ms/win) \\
\midrule
AMP (base) & 90.37 & 95.17 & 0.9713 & 4.19 $\pm$ 0.008 & 4.24 $\pm$ 0.008 & 6.99 $\pm$ 0.010 \\
INT8       & 48.74 & 95.30 & 0.9700 & 5.08 $\pm$ 0.002 & 5.13 $\pm$ 0.002 & 7.86 $\pm$ 0.005 \\
INT4       & 41.80 & 95.35 & 0.9743 & 4.47 $\pm$ 0.002 & 4.51 $\pm$ 0.002 & 7.25 $\pm$ 0.009 \\
\bottomrule
\end{tabular*}
\end{table}

\subsection{Efficiency benchmark}
\label{sec:eff}
We benchmark inference on an NVIDIA L4 GPU using 12\,s windows, batch size 1 (streaming). Table~\ref{tab:eff} reports parameters, checkpoint size, latency, and real-time factor (RTF).

\begin{table}[t]
\centering
\caption{Efficiency on NVIDIA L4 (12\,s windows, batch 1).}
\label{tab:eff}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr}
\toprule
Backbone & Params(M) & MB & ms & RTF \\
\midrule
DistilHuBERT & 23.49 & 93.97 & 6.72 & 5.60e-4 \\
Distil-wav2vec2 & 51.84 & 207.52 & 8.11 & 6.76e-4 \\
HuBERT Base & 94.37 & 377.57 & 10.05 & 8.37e-4 \\
wav2vec2 Base & 94.37 & 377.61 & 9.99 & 8.33e-4 \\
WavLM Base+ & 94.38 & 377.62 & 18.31 & 1.53e-3 \\
\bottomrule
\end{tabular*}
\end{table}

% \begin{table}[t]
\begin{table}[H]
\centering
\caption{Per-language and overall classification performance (scripted = 1, spontaneous = 0).}
\label{tab:results}
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrr}
\toprule
Language & n & Acc & AUC & TN & FP & FN & TP \\
\midrule
bas & 1793 & 0.8762 & 0.9411 & 335 & 81 & 141 & 1236 \\
gl  & 839  & 0.7843 & 0.8422 & 159 & 44 & 137 & 499 \\
qxp & 3871 & 0.7316 & 0.7384 & 767 & 281 & 758 & 2065 \\
ru  & 1700 & 0.7553 & 0.7013 & 292 & 94 & 322 & 992 \\
tr  & 139  & 0.7410 & 0.6496 & 21  & 7  & 29  & 82 \\
\midrule
Overall & 8342 & 0.7730 & 0.7365 & 1574 & 507 & 1387 & 4874 \\
\bottomrule
\end{tabular*}
\end{table}

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{fig_backbone_deployment_profile.png}
  \caption{Backbone deployment profile on NVIDIA L4: parameter count, checkpoint size, and streaming latency for 12\,s windows at batch size 1.}
  \label{fig:efficiency}
\end{figure}

\FloatBarrier


